Multi-Objective Hyperparameter Optimization in Machine Learning -- An Overview

Hyperparameter optimization constitutes a large part of typical modern machine learning workflows. This arises from the fact that machine learning methods and corresponding preprocessing steps often only yield optimal performance when hyperparameters are properly tuned. But in many applications, we are not only interested in optimizing ML pipelines solely for predictive accuracy; additional metrics or constraints must be considered when determining an optimal configuration, resulting in a multi-objective optimization problem. This is often neglected in practice, due to a lack of knowledge and readily available software implementations for multi-objective hyperparameter optimization. In this work, we introduce the reader to the basics of multi-objective hyperparameter optimization and motivate its usefulness in applied ML. Furthermore, we provide an extensive survey of existing optimization strategies, both from the domain of evolutionary algorithms and Bayesian optimization. We illustrate the utility of MOO in several specific ML applications, considering objectives such as operating conditions, prediction time, sparseness, fairness, interpretability and robustness.

==> figures/applications_taxonomy.tex <==
\begin{tikzpicture}[scale=0.5, every node/.style={transform shape},
    shorten >=0.5pt, >={Stealth[round]},
    hbox/.style = {rectangle, rounded corners = 2, node distance = 2.5cm, fill = white, draw = black, thick, text width = 9em, align = center,
        blur shadow = {shadow blur steps = 5}, minimum height = 1cm, minimum width = 1.5cm, font = \large
},
    sbox/.style = {rectangle, rounded corners = 2, node distance = 1.5cm, fill = white, draw = black, thick, text width = 8em, align = center,
        blur shadow = {shadow blur steps = 5}, minimum height = 1cm, minimum width = 1.5cm
}]

%% Headers
% nodes
\node[hbox, text width = 12em] (application) at (0, 0) {Application Domains};
\node[hbox, below of = application, xshift = -12.5cm] (performance) {Performance};
\node[hbox, below of = application, xshift = -7.5cm] (efficiency) {Efficiency};
\node[hbox, below of = application, xshift = -2.5cm] (fairness) {Fairness};
\node[hbox, below of = application, xshift = 2.5cm] (interpretability) {Interpretability};
\node[hbox, below of = application, xshift = 7.5cm] (robustness) {Robustness};
\node[hbox, below of = application, xshift = 12.5cm] (sparseness) {Sparseness};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (performance.north |- , -1)  -- (performance.north);
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (efficiency.north |- , -1)  -- (efficiency.north);
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (fairness.north |- , -1)  -- (fairness.north);
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (interpretability.north |- , -1)  -- (interpretability.north);
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (robustness.north |- , -1)  -- (robustness.north);
\draw[-narrowtriangle, line width = 0.3mm, black] (application.south) -- (0, -1) -- (sparseness.north |- , -1)  -- (sparseness.north);

%% Performance
% nodes
\node[sbox, below right of = performance, yshift = -1.5cm] (roc) {ROC Analysis};
\node[sbox, below right of = performance, yshift = -3.5cm] (nlp) {Natural Language Processing};
\node[sbox, below right of = performance, yshift = -5.5cm] (dots) {$\ldots$};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (performance.text |- performance.south) |- (roc.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (performance.text |- performance.south) |- (nlp.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (performance.text |- performance.south) |- (dots.west);

%% Efficiency
% nodes
\node[sbox, below right of = efficiency, yshift = -1.5cm] (flop){Energy\\Consumption};
\node[sbox, below right of = efficiency, yshift = -3.5cm] (model){Memory\\Consumption};
\node[sbox, below right of = efficiency, yshift = -5.5cm] (inference){Prediction and Training Time};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (efficiency.text |- efficiency.south) |- (flop.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (efficiency.text |- efficiency.south) |- (model.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (efficiency.text |- efficiency.south) |- (inference.west);

%% Fairness
% nodes
\node[sbox, below right of = fairness, yshift = -1.5cm] (odds) {Equalized Odds};
\node[sbox, below right of = fairness, yshift = -3.5cm] (opps) {Equality of Oppurtunity};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (fairness.text |- fairness.south) |- (odds.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (fairness.text |- fairness.south) |- (opps.west);

%% Interpretability
% nodes
\node[sbox, below right of = interpretability, yshift = -1.5cm] (spar) {Sparseness};
\node[sbox, below right of = interpretability, yshift = -3.5cm] (int) {Interaction Strength};
\node[sbox, below right of = interpretability, yshift = -5.5cm] (comp) {Complexity of Main Effects};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (interpretability.text |- interpretability.south) |- (spar.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (interpretability.text |- interpretability.south) |- (int.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (interpretability.text |- interpretability.south) |- (comp.west);

%% Robustness
% nodes
\node[sbox, below right of = robustness, yshift = -1.5cm] (dom) {Distribution Shift};
\node[sbox, below right of = robustness, yshift = -3.5cm] (adv) {Adversarial Examples};
\node[sbox, below right of = robustness, yshift = -5.5cm] (pert) {Perturbations};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (robustness.text |- robustness.south) |- (dom.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (robustness.text |- robustness.south) |- (adv.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (robustness.text |- robustness.south) |- (pert.west);

%% Sparseness
% nodes
\node[sbox, below right of = sparseness, yshift = -1.5cm] (nfeat) {Number of Features};
\node[sbox, below right of = sparseness, yshift = -3.5cm] (feats) {Stability of Feature Seletion};
% arrows
\draw[-narrowtriangle, line width = 0.3mm, black] (sparseness.text |- sparseness.south) |- (nfeat.west);
\draw[-narrowtriangle, line width = 0.3mm, black] (sparseness.text |- sparseness.south) |- (feats.west);

%% FAT-ML
\draw[draw = green!60!black, dashed, line width = 1.5, rounded corners = 4] (14.7, -10.6) -- (15.5, -10.6) -- (15.5, -1.5) -- (-4.5, -1.5) -- (-4.5, -10.6) -- (7.8, -10.6);
\node[font = \Large, fill = none] at (11.24, -10.6) [text = green!60!black] {\textbf{FAT-ML related objectives}};
\end{tikzpicture}

==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(x)}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{\tilde{r}^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{\tilde{r}^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}


==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}


==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
\newcommand{\HS}{\Phi}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


\newcommand{\alphah}{\hat{\alpha}}													% alpha-hat
\newcommand{\alphav}{\bm{\alpha}}													% vector alpha (bold)
\newcommand{\alphavh}{\hat{\bm{\alpha}}}													% vector alpha-hat



\newcommand{\phix}{\phi(\xv)}          												% \phi(x)
\newcommand{\phixt}{\phi(\tilde \xv)}        										% \phi(x-tilde)



==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}


==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

